A Survey on Centrality and Importance Measures in Hypergraphs: Categorization and Empirical Insights

Identifying central entities and interactions is a fundamental problem in network science. While well-studied for graphs (pairwise relations), many biological and social systems exhibit higher-order interactions best modeled by hypergraphs. This has led to a proliferation of specialized hypergraph centrality measures, but the field remains fragmented and lacks a unifying framework. This paper addresses this gap by providing the first systematic survey of 39 distinct measures. We introduce a novel taxonomy classifying them as: (1) structural (topology-based), (2) functional (impact on system dynamics), or (3) contextual (incorporating external features). We also present an experimental assessment comparing their empirical similarity and computation time. Finally, we discuss applications, establishing a coherent roadmap for future research in this area.

==> dfn.tex <==
\RequirePackage{tikz}
\RequirePackage[edges]{forest}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{tikzmark}
\usetikzlibrary{bending}
\RequirePackage{multicol}
\usetikzlibrary{shadows}
\RequirePackage{tikz-qtree}
\usetikzlibrary{shadows.blur}
\usepackage{xcolor}
\usepackage{makecell}
\usepackage{bigstrut}
\usepackage{array}
\usepackage{graphicx}
\usepackage{collcell}
\newcommand{\ScaleCell}[1]{\scalebox{0.9}{#1}}

%\newcommand{\red}{\textcolor{red}}

\newcommand{\smallsection}[1]{{\noindent {\bf{\underline{\smash{#1}}}}}}

\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\boldsymbol{\rm #1}}
\newcommand{\matt}[1]{\mathbf{#1}^{\top}}
\newcommand{\matd}[1]{\mathbf{\tilde{#1}}}
\newcommand{\mati}[1]{\mathbf{#1}^{-1}}
\newcommand{\mattt}[1]{\mathbf{\tilde{#1}}^{\top}}

\newcommand{\nnz}[1]{\texttt{nnz}(#1)}

% Define softer colors
\definecolor{softgreen}{RGB}{0,128,0}   % Darker, more readable green
\definecolor{softred}{RGB}{178,34,34}   % Firebrick red

% New commands using the softer colors
\newcommand{\cmark}{\textcolor{softgreen}{\ding{51}}}  % ✓
\newcommand{\xmark}{\textcolor{softred}{\ding{55}}}    % ✗

\newcommand{\vdep}{\textit{Var.}}
\newcommand{\mdep}{\textit{Model}}

\usepackage[capitalise]{cleveref}
 
\makeatletter
% #1 = internal counter name
% #2 = printed prefix (e.g. “P”, “E”)
\newcommand{\NewNumberedSection}[2]{%
  \newcounter{#1}%
  \setcounter{#1}{0}%
  % \foo{Title}
  \expandafter\newcommand\csname #1\endcsname[1]{%
    \refstepcounter{#1}%
    \smallsection{#2\csname the#1\endcsname. ##1}%
  }%
  % \foo ref
  \expandafter\newcommand\csname #1ref\endcsname[1]{%
    #2\ref{##1}\xspace%
  }%
  % cleveref integration
  \crefname{#1}{}{}%   singular and plural form both “P” or “E”
  \Crefname{#1}{}{}%   same for capitalized \Cref
  \creflabelformat{#1}{##2#2##1##3}%  make \cref print “P⟨num⟩”
}
\makeatother

% define your two types
\NewNumberedSection{prelim}{P}
\NewNumberedSection{element}{E}
\NewNumberedSection{centrality}{M}



\usepackage[most]{tcolorbox}

\newcounter{discussion}
\renewcommand{\thediscussion}{\arabic{discussion}}



\tcbset{
  discussionbox/.style={
    colback=gray!10,
    colframe=black!50,
    boxrule=0.5pt,
    arc=3pt,
    left=2mm,
    right=2mm,
    top=1mm,
    bottom=1mm,
    fonttitle=\bfseries,
  }
}

\newenvironment{discussion}[1][]{%
  \begin{tcolorbox}[discussionbox,title=#1]%
}{%
  \end{tcolorbox}%
}

